Cloud K-SVD: A Collaborative Dictionary Learning Algorithm for Big, Distributed Data

This paper studies the problem of data-adaptive representations for big, distributed data. It is assumed that a number of geographically-distributed, interconnected sites have massive local data and they are interested in collaboratively learning a low-dimensional geometric structure underlying these data. In contrast to previous works on subspace-based data representations, this paper focuses on the geometric structure of a union of subspaces (UoS). In this regard, it proposes a distributed algorithm---termed cloud K-SVD---for collaborative learning of a UoS structure underlying distributed data of interest. The goal of cloud K-SVD is to learn a common overcomplete dictionary at each individual site such that every sample in the distributed data can be represented through a small number of atoms of the learned dictionary. Cloud K-SVD accomplishes this goal without requiring exchange of individual samples between sites. This makes it suitable for applications where sharing of raw data is discouraged due to either privacy concerns or large volumes of data. This paper also provides an analysis of cloud K-SVD that gives insights into its properties as well as deviations of the dictionaries learned at individual sites from a centralized solution in terms of different measures of local/global data and topology of interconnections. Finally, the paper numerically illustrates the efficacy of cloud K-SVD on real and synthetic distributed data.

==> docs/NumericalEvaluation.tex <==
\section{Numerical Experiments}\label{section:NumericalEvaluation}
We present numerical results in this section for demonstrating
the usefulness of cloud K-SVD and also validating some of our theoretical results. In the first set of experiments, synthetic data is used to demonstrate efficacy of cloud $K$-SVD for data representation. Furthermore, behavior of distributed power method (Steps~7--17 in Algorithm~\ref{algo:Distributed_KSVD}) as a function of the number of consensus iterations and deviations in cloud $K$-SVD dictionaries from centralized dictionary as a function of number of power method iterations are also shown with the help of simulations. In the second set of experiments, MNIST dataset is used to motivate an application of cloud $K$-SVD that can benefit from collaborations between distributed sites.
%
%We perform two kinds of numerical simulations. First, in
%subsection~\ref{subsec:syntheticData} we will perform some experiments on
%synthetic data to demonstrate the working of cloud K-SVD, and how different
%parameters effect convergence of algorithm. Then in
%subsection~\ref{subsec:realData} we will demonstrate the efficacy of cloud
%K-SVD for classification of MNIST dataset.
\subsection{Experiments Using Synthetic Data}
\label{subsec:syntheticData} These experiments correspond to a total of $N = 100$ sites, with each site having $S_i = 500$ local samples in $\mathbb{R}^{20}$ (i.e., $n = 20$). Interconnections between the sites are
randomly generated using an Erd\H{o}s--R\'{e}nyi graph with parameter
$p=0.5$. In order to generate synthetic data at individual sites, we first
generate a dictionary with $K=50$ atoms, $\Dictionary \in \mathbb{R}^{20 \times 50}$, with columns uniformly distributed on the unit sphere in $\mathbb{R}^{20}$. Next,
we randomly select a $45$-column subdictionary of $\Dictionary$ for each site
and then generate samples for that site using a linear combination of $T_0 =
3$ randomly selected atoms of this subdictionary, followed by addition of
white Gaussian noise with variance $\sigma^2 = 0.01$. All data samples in our
experiments are also normalized to have unit $\ell_2$ norms. Finally, in
order to carry out distributed consensus averaging, we generate a
doubly-stochastic weight matrix $W$ according to the local-degree weights
method described in \cite[Sec.~4.2]{xiao2004fast}. For estimating eigenvectors during dictionary update step using distributed power method we use $T_p=15$ power method iterations and $T_c=15$ consensus iterations.

Based on above setup our first set of experiments demonstrate the effectiveness of collaboratively learning a dictionary using cloud K-SVD, as opposed to each site learning a \emph{local
dictionary} from its local data using the canonical K-SVD algorithm (referred
to as \emph{local K-SVD} in the following). In
Fig.~\ref{fig:RepresentationError}, we plot average representation error,
defined as $\frac{1}{n S}\sum_{i=1}^{N}{\sum_{j=1}^{S_i}{\|y_{i,j} - D
x_{i,j}\|_2}}$, as a function of the number of dictionary learning iterations
for three dictionary learning methods, namely, centralized (canonical) K-SVD,
cloud K-SVD, and local K-SVD. It can be seen from this figure, which
corresponds to an average of 100 Monte-Carlo trials, that cloud K-SVD and centralized $K$-SVD have similar performance and both of them perform better than local K-SVD. In particular, the local K-SVD error is $\approx 0.06$ after 50 iterations, while it is $\approx 0.03$ for cloud K-SVD and centralized K-SVD.

\begin{figure}[t]%
\centering
\includegraphics[width=0.4\columnwidth]{./Figures/ReconstructionError.png}%
\caption{Average representation error as a function of the number of dictionary learning iterations for centralized K-SVD, cloud K-SVD, and local K-SVD.}%
\label{fig:RepresentationError}%
\vspace{-1.5\baselineskip}%
\end{figure}

The second set of experiments that we perform illustrate the convergence
behavior of the distributed power method within cloud K-SVD (Steps 7--17 in
Algorithm~\ref{algo:Distributed_KSVD}) as a function of the number of
consensus iterations. The results of these experiments, which are reported in
Fig.~\ref{fig:DistributedPowerMethod}, correspond to five different values of
the number of consensus iterations (3, 4, 5, 10, 15) within each iteration of
the distributed power method. Specifically, let $q$ denote the
principal eigenvector of the matrix $\widehat{M}$ in
Algorithm~\ref{algo:Distributed_KSVD} computed using Matlab and $\widehat{q}_1^{(t_p)}$ denote an estimate of $q$ obtained at site $1$ in iteration $t_p$ using
the distributed power method. Then Fig.~\ref{fig:DistributedPowerMethod} plots
$\|q q^\tT - \widehat{q}_1^{(t_p)}{\widehat{q}_1^{(t_p)
\tT}}\|_2$ averaged over all distributed power method iterations, dictionary
learning iterations, and 100 Monte-Carlo trials as a function of the number
of distributed power method iterations. It can be seen from this figure that
the distributed power method hits an \emph{error floor} with increasing number of
distributed power method iterations, where the floor is fundamentally
determined by the number of consensus iterations, as predicted by
Theorem~\ref{theorem:DistributedPowerMethod}.

Our third experiment highlights the average error in dictionary atoms learned
using cloud K-SVD as compared to centralized K-SVD. Experimental setup is
still the same as in first experiment. For this experiment number of consensus iterations $T_c$ are fixed to~15, while the number of power method iterations $T_p$ correspond to 2, 3, 4 and 5 to show the effect of $T_p$ on error in collaborative dictionaries as compared to centralized K-SVD. Error in dictionary atoms is averaged over all the atoms and sites for 100 Monte-Carlo trials, and error in each trial can be mathematically written as $E_{\text{average}}^{(t)}=\frac{1}{NK}\sum_{k=1}^{K}\sum_{i=1}^{N}{\|d_k^{(t)} d_k^{(t)^{\tT}} - \widehat{d}_{i,k}^{(t)} \widehat{d}_{i,k}^{(t)^{\tT}}\|_2}$. Simulation results in Fig.~\ref{fig:DictionaryErrorVaryingPowerIterations} show that error in dictionary atoms increases sharply at the start and after some iterations error becomes stable. Important point to note here is that as we increase the number of power method iterations we get smaller average error in dictionary atoms as predicted by our analysis. {\color{red}On the other hand Fig.~\ref{fig:RepresentationErrorVaryingPowerIterations} shows that decreasing power method iterations has no impact on representation error.}

\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{0.4\columnwidth}
	\centering
		\includegraphics[width=\textwidth]{./Figures/DictionaryError.png}
		\caption{Dictionary error.}
		\label{fig:DictionaryErrorVaryingPowerIterations}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.4\columnwidth}
	\centering
	\includegraphics[width=\textwidth]{./Figures/RepresentationErrorVaryingPowerIterations.png}%
	\caption{Representation error.}
	\label{fig:RepresentationErrorVaryingPowerIterations}
	\end{subfigure}
		\caption{Average error in dictionary atoms and representation errors as a function of dictionary learning iteration for different values of power method iterations ($T_p$).}
		\vspace{-1.5\baselineskip}
\end{figure}

{\color{red}Next we provide performance of K-SVD for online settings in terms of representation error. Data generation process is still the same as described in first paragraph of this section. A batch of 500 training samples is generated periodically. We assume that we have a buffer limit of 1000 samples, therefore only the samples from last two are used for dictionary learning. Note that further improvements in learning can be achieved by using other methods like [cite Tong's latest work here] for selection of training samples. Dictionary learned at previous interval is used to warm restart K-SVD and 60 dictionary learning iterations are performed. Fig.~\ref{fig:OnlineKSVD} shows the representation error for six periods as a function of dictionary learning iterations. Ending of a period is marked by a black circle in Fig.~\ref{fig:OnlineKSVD}. We can see that for first period K-SVD takes more time to converge than the other periods.}
\begin{figure}%
\centering
\includegraphics[width=0.4\columnwidth]{Figures/OnlineKSVD}%
\caption{Performance of K-SVD for online settings.}%
\vspace{-\baselineskip}
\label{fig:OnlineKSVD}%
\end{figure}

{\color{red}Finally we perform simulations to compute analysis parameters $C_1-C_4$. For these simulations we generate samples belonging to $\mathbb{R}^{17}$ and each sample is a linear combination of $T_0=3$ atoms of a dictionary $D\in\mathbb{R}^{17\times 40}$. For this simulation we are using Lasso package from MATLAB. For this setup we perform dictionary learning using K-SVD and average values obtained for parameters $C_1-C_4$ over 100 Monte-Carlo trials are 0.0586, 0.1633, 4.544, and 1.5947 respectively. Using cloud K-SVD average values of $\mu$ and $\nu$ are 9000 and 0.3242 respectively. Based on these values we get $T_p\approx 16,000$. This shows the looseness of our bounds and also that our analysis is useful when doing asymptotic comparisons.}
\begin{figure}[t]%
\centering
\includegraphics[width=0.4\columnwidth]{./Figures/DistributedPowerMethod.eps}%
\caption{Convergence behavior of the distributed power method as a function of varying number of consensus averaging iterations.}%
\label{fig:DistributedPowerMethod}%
\vspace{-0.5\baselineskip}%
\end{figure}

\subsection{{\color{red}Classification of MNIST Images}}
\label{subsec:realData}
\begin{figure}[t]
	\centering
		\includegraphics[width=0.4\columnwidth]{./Figures/Classification_MNIST_Chainais.png}
	\caption{Average detection rate for five classes of MNIST dataset using centralized K-SVD, cloud K-SVD, method by~\cite{chainais2013learning}, and local K-SVD.}
	\vspace{-1.5\baselineskip}
	\label{fig:Classification_MNIST}
\end{figure}
For evaluation of cloud K-SVD for real dataset, we perform classification of
digits $\{0, 3, 5, 8, 9\}$ from MNIST dataset~\cite{mnist-database}. For each
digit~6000 samples are used, where~5000 samples are used for training
purposes and remaining~1000 for testing. Furthermore, the data are five-times
randomly split into training and test samples. For cloud $K$-SVD {\color{red}and method in~\cite{chainais2013learning}},
Erd\H{o}s--R\'{e}nyi graph with parameter $p=0.5$ is used to generate a
network with~10 sites and data is equally distributed among these $10$ sites.
Before performing dictionary learning, data is down sampled from
$\mathbb{R}^{784}$ to $\mathbb{R}^{256}$. After downsampling, a separate
dictionary is learned for each digit using centralized K-SVD, cloud K-SVD{\color{red}, ~\cite{chainais2013learning}'s method},
and K-SVD using only local data. Each dictionary has dimensions
$\mathbb{R}^{256\times 400}$, i.e., $K=400$, and sparsity level of 10 is
used, i.e., $T_0=10$. Minimum residue based
rule~\cite[Sec.II-A]{chen2011hyperspectral} is used for classification, more
details on which are given in the following paragraph.

Let $\{D_c\}_{c=1}^{5}$ be the set of dictionaries for~5 classes and let $D=\begin{bmatrix} D_1 & D_2 & D_3 & D_4 & D_5\end{bmatrix}$ be the complete dictionary. For any test sample $y_s$, we perform sparse coding using dictionary $D$ with sparsity constraint of $T_0=10$ to get coefficients $x_s\in \mathbb{R}^{2000}$. Then we partition $x_s$ into five segment $\{x_{s,c}\}_{c=1}^{5}$, where $x_{s,c}$ are the coefficients corresponding to dictionary $D_c$ of class $c$. Next we define residue for class $c$ as $r_c = \|y_s - D_c x_{s,c}\|_2$. Finally, the detected class is given by $c^{*}=\arg\min_{c}{r_c}$. Performance of each method (centralized $K$-SVD, cloud $K$-SVD{\color{red}, method in~\cite{chainais2013learning}}, and local $K$-SVD) is measured in terms of average detection rate on the test samples, which is defined as,
$$R_c = \frac{\text{Number of samples in class }c\text{ detected correctly}}{\text{Total number of samples of class } c}.$$
Results of this experiment are given in Figure~\ref{fig:Classification_MNIST}. We can see that centralized $K$-SVD and cloud $K$-SVD have comparable
performance. While in the case of local $K$-SVD where we only use the local data
for learning representations, classification rate deteriorates
considerably. {\color{red}Moreover, we can see that distributed dictionary learning method proposed by~\cite{chainais2013learning} performs poorly}. The bars in local $K$-SVD show the highest and lowest detection rates achieved among the $10$~sites, which highlights the variation in effectiveness of models learned across different sites when using only the local data.
